Tuning contact angles of aqueous droplets on hydrophilic and hydrophobic surfaces by surfactants

Adsorption of small amphiphilic molecules occurs in various biological and technological processes, sometimes desired, the other times unwanted (e.g., contamination). Surface-active molecules preferentially bind to interfaces and affect their wetting properties. We study the adsorption of short-chained alcohols (simple surfactants) to the water-vapor interface and solid surfaces of various polarities using molecular dynamics simulations. The analysis enables us to establish a theoretical expression for the adsorption coefficient, which exponentially scales with the molecular surface area and the surface wetting coefficient, and which is in good agreement with the simulation results. The competition of the adsorptions to both interfaces of a sessile droplet alters its contact angle in a nontrivial way. The influence of surfactants is strongest on very hydrophilic and very hydrophobic surfaces, whereas droplets on surfaces of moderate hydrophilicity are much less affected.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc_old <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
